A Central Limit Theorem for Differentially Private Query Answering

Perhaps the single most important use case for differential privacy is to privately answer numerical queries, which is usually achieved by adding noise to the answer vector. The central question, therefore, is to understand which noise distribution optimizes the privacy-accuracy trade-off, especially when the dimension of the answer vector is high. Accordingly, extensive literature has been dedicated to the question and the upper and lower bounds have been matched up to constant factors [BUV18, SU17]. In this paper, we take a novel approach to address this important optimality question. We first demonstrate an intriguing central limit theorem phenomenon in the high-dimensional regime. More precisely, we prove that a mechanism is approximately Gaussian Differentially Private [DRS21] if the added noise satisfies certain conditions. In particular, densities proportional to $\mathrm{e}^{-\|x\|_p^\alpha}$, where $\|x\|_p$ is the standard $\ell_p$-norm, satisfies the conditions. Taking this perspective, we make use of the Cramer--Rao inequality and show an "uncertainty principle"-style result: the product of the privacy parameter and the $\ell_2$-loss of the mechanism is lower bounded by the dimension. Furthermore, the Gaussian mechanism achieves the constant-sharp optimal privacy-accuracy trade-off among all such noises. Our findings are corroborated by numerical experiments.

==> ROC.tex <==
\newcommand{\Lap}{\mathrm{Lap}}
\section{GDP and the ROC functions} % (fold)
\label{sec:gdp_and_the_roc_functions}
Let $\xi$ be a two-sided geometric random variable with parameter $p\in(0,1)$ (see e.g. \cite{ghosh2012universally}). That is, it supports on integers and 
$\P(\xi=n)=\frac{1-p}{1+p}\cdot p^{|n|}$. Take an independent random variable $U$ with uniform distribution on $[-\frac{1}{2},\frac{1}{2}]$. We denote the distribution of $\xi+U$ by $\mathrm{TGU}(p)$, which stands for ``Two-sided Geometric plus Uniform''.\\
For $h>0$, let $\Lap^h(0,1)$ be standard Laplace truncated at $\pm h$. Its density is
$\frac{1_{|x|<h}}{1-\e^{-h}}\cdot\frac{1}{2}\e^{-|x|}$.

In the following we use the simplified notation $T_X=T[X,X+1]$. In particular, $T_X\geqslant f_{\ep,\delta}$ if and only if adding noise $X$ to a sensitivity 1 query is $(\ep,\delta)$-DP.
\begin{lemma}\label{lem:ROCtable}
	\begin{enumerate}
		\item For $X=\ep^{-1}\cdot\Lap(0,1)$, $\E X^2 =\frac{2}{\ep^2}$ and
		$T_X=f_{\ep,0}$ except on the interval $[\tfrac{1}{2}\e^{-\ep},\tfrac{1}{2}]$. On that interval, it is a reciprocal function, namely
\begin{align*}
	\alpha\cdot T_X(\alpha)=
		\e^{-\ep}/4, \alpha\in[\tfrac{1}{2}\e^{-\ep},\tfrac{1}{2}].
	% \left\{
	% \begin{array}{ll}
	% 	% 1-\e^{\ep}\alpha, 		& \alpha < \e^{-\ep}/2, \\
	% 	f_{\ep,0},& x\not\in,\\
	% 	% \e^{-\ep}(1-\alpha), & \alpha>1/2.
	% \end{array}
	% \right.
\end{align*}
In particular, $\|T_X-f_{\ep,0}\|_\infty=O(\ep^2)$ as $\ep\to0$.
		\item For $X=\mathrm{TGU}(\e^{-\ep})$, $\E X^2 =\frac{1}{2\sinh^2{\frac{\ep}{2}}}+\frac{1}{12}=\frac{2}{\ep^2}+O(1)$  when $\ep\to 0$ and $T_X=f_{\ep,0}$
		\item For $X=\ep^{-1}\cdot N(0,1)$, $\E X^2 =\frac{1}{\ep^2}$ and $T_X=G_{\ep}$
		\item For $X=\ep^{-1}\cdot \Lap^h(0,1)$ with $h=\log (1+\frac{\e^\ep-1}{2\delta})$, $\E X^2 =\frac{2}{\ep^2}\cdot\left(1-\frac{\ep^2h(h+2)}{\e^h-1}\right)$ and $T_X=f_{\ep,\delta}$ except on the interval $[(\tfrac{1}{2}-\delta)\e^{-\ep},\tfrac{1}{2}]$. On that interval, it is conjugate via a linear function to a reciprocal function, namely
\begin{align*}
	L_h(\alpha)\cdot L_h\big(T_X(\alpha)\big)=
		\e^{-\ep}/4, \alpha\in[(\tfrac{1}{2}-\delta)\e^{-\ep},\tfrac{1}{2}].
	% \left\{
	% \begin{array}{ll}
	% 	% 1-\e^{\ep}\alpha, 		& \alpha < \e^{-\ep}/2, \\
	% 	f_{\ep,0},& x\not\in,\\
	% 	% \e^{-\ep}(1-\alpha), & \alpha>1/2.
	% \end{array}
	% \right.
\end{align*}
where $L_h(x) = (1-\e^{-h})x+\frac{1}{2}\e^{-h}$.
In particular, $\E X^2 =\frac{2}{\ep^2}+O(1)$ and $\|T_X-f_{\ep,\delta}\|_\infty=O(\ep^2)$ when $\delta<\frac{\ep}{2}$ and $\ep\to0$.
% \begin{align*}
% 	T_X(\alpha)=
% 	\left\{
% 	\begin{array}{ll}
% 		% 1-\e^{\ep}\alpha, 		& \alpha < \e^{-\ep}/2, \\
% 		f_{\ep,\delta},& x\not\in[\e^{-\ep}(\tfrac{1}{2}-\delta),\tfrac{1}{2}]\\
% 		\e^{-\ep}/4\alpha, &x\in[\e^{-\ep}(\tfrac{1}{2}-\delta),\tfrac{1}{2}]
% 		% \e^{-\ep}(1-\alpha), & \alpha>1/2.
% 	\end{array}
% 	\right.
% \end{align*}
	\end{enumerate}
\end{lemma}
\input{ROC_table}
As we see in the variance column, $2\log(1.25\delta^{-1})$ is the only factor that blows up to infinity, while the others differ by a factor of at most 2. Therefore, all but the last row are more or less acceptable. This suggests, in some sense, Gaussian mechanism and $(\ep,\delta)$-DP are quite a mismatch and should not be applied together in applications where optimizing the constant is a concern.

TGU mechanism is a special case of the staircase mechanism in \cite{geng2014optimal}. In fact, $\mathrm{TGU}(\e^{-\ep})$ is exactly the $\mathcal{P}_\gamma$ distribution (defined in equation (37) of \cite{geng2014optimal}) with $\gamma=\frac{1}{2}$ and $\Delta=1$. Their Theorem 6 shows that adding noise $\mathcal{P}_\gamma$ with a specific $\gamma$ achieves minimal variance among all noise addition mechanisms that are $(\ep,0)$-DP, where this optimal parameter $\gamma^*$ depends on $\e^{-\ep}$ in a complicated way. However, $\mathrm{TGU}(\e^{-\ep})$ is very close to optimal. As is shown in our \Cref{lem:ROCtable} and their Corollary 7, both $\mathrm{TGU}(\e^{-\ep})$ and $\mathcal{P}_\gamma$ have variance $\frac{2}{\ep^2}-O(1)$. In fact, using the exact expressions provided in these two results, we can show that $\mathrm{TGU}(\e^{-\ep})$ has variance at most $0.3\%$ larger than the optimum when $\ep\leqslant 1$.
\begin{proof}[Proof of \Cref{lem:ROCtable}]
\begin{enumerate}
	\item The expression of $T_X$ is determined in Lemma A.6
\end{enumerate}
By Wolfram Alpha $\sum_{n\geqslant1}n^2p^n = \frac{p(p+1)}{(1-p)^3}$. So if $\xi\sim\mathrm{DGeom}(p)$ then
	\[\E\xi^2 = \frac{2}{Z}\sum_{n\geqslant1}n^2p^n = 2\cdot\frac{1-p}{1+p}\cdot\frac{p(p+1)}{(1-p)^3}=\frac{2p}{(1-p)^2}=\frac{2}{(\e^{\frac{\ep}{2}}-\e^{-\frac{\ep}{2}})^2}=\frac{1}{2\sinh^2{\frac{\ep}{2}}}\leqslant \frac{2}{\ep^2}.\]
$X$ has log-concave density and cdf $F$. It was shown in Proposition A.3 of \cite{dong2019gaussian} that $T[X,X+t](\alpha)=F(F^{-1}(1-\alpha)-t)$


% Consider discrete distributions $P,Q$ on a countable probability space. WLOG assume the domain is $\mathbb{N}$(or $\Z$). The probability mass are $\{p_i\}_{i\geqslant 1}$ and $\{q_i\}_{i\geqslant 1}$ respectively. Consider two functions
% \begin{align*}
% 	\alpha(h)&:=\sum_{\{i:\log \frac{q_i}{p_i}>h\}} p_i\\
% 	\beta(h)&:=\sum_{\{i:\log \frac{q_i}{p_i}\leqslant h\}} q_i
% \end{align*}
% For each $h$, the set $\{i:\log \frac{q_i}{p_i}>h\}$ is a subset of $\mathbb{N}$, hence the summation is over a subsequence of $\{p_i\}_{i\geqslant 1}$. The range of the two functions are subsets of $[0,1]$. The range of $h\mapsto (\alpha(h),\beta(h))$ is a countable subset of $[0,1]^2$.
% The graph of $T[P,Q]$ is the convex hull of this set. For a given $x$, if $\mathrm{ran} \alpha \cap [0,x]$ has a maximum and $\mathrm{ran} \alpha \cap[x,1]$ has a minimum, then $T[P,Q](x)$ can be determined. In general it's tricky. In particular, it is not always possible to order the values $\log \frac{q_i}{p_i}$. In fact, it is impossible if the set of $\log \frac{q_i}{p_i}$ has two limit points, say the set $\{1+\frac{1}{n}\}_{n\geqslant 1}\cup\{2+\frac{1}{n}\}_{n\geqslant 1}$.


	\[\frac{\e^{-\ep}}{4}\cdot(1+\e^\ep)-\frac{1}{1+\e^\ep}=\frac{1+\e^{-\ep}}{4}-\frac{1}{1+\e^\ep}=\frac{\e^\ep+\e^{-\ep}-2}{4(1+\e^\ep)}=O(\ep^2)=o(\ep)\]
	\begin{align*}
	new diff = L_h^{-1}(\frac{1+\e^{-\ep}}{4})-L_h^{-1}(\frac{1}{1+\e^\ep})
	\end{align*}
	$L_h^{-1}(x)=\frac{x-\frac{1}{2}\e^{-h}}{1-\e^{-h}}$
	so $new diff = \frac{1}{1-\e^{-h}} old diff$. and
	$\frac{1}{1-\e^{-h}}=\frac{2\delta}{\e^{\ep}-1}+1$ so old diff
	\begin{align*}
	=(\frac{2\delta}{\e^{\ep}-1}+1)\cdot\frac{\e^\ep+\e^{-\ep}-2}{4(1+\e^\ep)}=(\frac{2\delta}{\e^{\ep}-1}+1)\cdot O(\ep^2)
	\end{align*}
	So if $2\delta<\ep<\e^\ep-1$, we have old diff $=O(\ep^2)$.
\end{proof}
\begin{enumerate}
	\item For $h>0$, let $\Lap^h$ be standard Laplace truncated at $\pm h$.
	\begin{lemma} \label{lem:}
		\djs{Not 100\% sure} When $\xi\sim P$ as in the above lemma,
		\begin{align*}
			\E\xi^2 &= \frac{2-\e^{-h}(h^2+2h+2)}{1-\e^{-h}}.
		\end{align*}
	\end{lemma}
\end{enumerate}

Suppose $f=T(P,P+t)$ where $P$ is log-concave, with cdf $F$. Then $f(\alpha) = F(F^{-1}(1-\alpha)-t)$. Let $P^h$ be $P$ after $\pm h$ truncation. Its cdf is
\[F^h(x) = \frac{F(x)-F(-h)}{F(h)-F(-h)}\Big[^1_0\]
where $\Big[^1_0$ means truncating at 0 and 1. $P^h$ is still log-concave. Let's find $f^h = T(P^h,P^h+t)$. For the rejection region $\{x>a\}$, its type I and type II error are
\begin{align*}
	\alpha &= 1-F^h(a) = 1-\frac{F(a)-F(-h)}{F(h)-F(-h)}\Big[^1_0\\
	\beta &= F^h(a-t) =\frac{F(a-t)-F(-h)}{F(h)-F(-h)}\Big[^1_0
\end{align*}
Ignore truncation at 0 and 1 for now. Let $Z = F(h)-F(-h)$. Then
\begin{align*}
	1-F(a) &= Z\alpha+1-F(h)\\
	F(a-t)&=Z\beta+F(-h)
\end{align*}
That is, if $\beta = f^h(\alpha)$, then
\begin{align*}
	Z\beta+F(-h) = f(Z\alpha+1-F(h)).
\end{align*}
Let $L_h(x)=\frac{x-F(-h)}{F(h)-F(-h)}$. We have $F^h=L_h\circ F$.
\begin{theorem} \label{thm:}
$f^h$ is an affine conjugate of $f$, i.e.,
	\[f^h=L_h\circ f\circ L_h^{-1}.\]
\end{theorem}
Truncation in high-dimensional case is hard. We will no longer have this nice property, since the rejection region is complicated. To see this, consider product of truncated laplace. The trade-off function is $\big(L_h^{-1}\circ f\circ L_h\big)^{\otimes n}$. It is unlikely that this is an affine conjugate of $f^{\otimes n}$.

Back to 1-dim, ideally we want to find $P$ and $h$ such that $f^h = f_{\ep,\delta}$. To start let's find an approximate version first. Let $P=\Lap$. We have $F(-h)=\frac{1}{2}\e^{-h}$ and $Z = 1-\e^{-h}$.

A necessary condition for $f^h=f_{\ep,\delta}$ is $f^h(0)=1-\delta$. Now that we have fixed $P=\Lap$, this leads us to the expression of $h$. The resulting $f^h$ mostly agrees with $f_{\ep,\delta}$. The following lemma precisely describes this property.
% section gdp_and_the_roc_functions (end)
\begin{lemma}
	If $P,Q$ support on integers, then $T[P,Q] = T[P+U,Q+U]$.
\end{lemma}
But $T[P,Q]$ could be very complicated.
\begin{proof}
	$I_n=[n-1/2,n+1/2]$
	\begin{align*}
		\int (q-\e^\ep p)_+
		&=\sum_n\int_{I_n} (q-\e^\ep p)_+ = 
		\sum_n (q_n-\e^\ep p_n)_+
	\end{align*}
\end{proof}

Let $f_t=1-T[X,X+tv]$ and $s,t>0$. If $X$ is one-dimensional log-concave, then we know $f_{s+t} = f_{s}\circ f_{t}$. In particular, this semi-group property implies $f_{s+t}\geqslant f_t$. In general, by group privacy lemma, we know $f_{s+t} \leqslant f_{s}\circ f_{t}$.
We know $f_{s+t}\geqslant f_t$ if $X$ is log-concave in Rn. But the semi-group property does not hold when dimension $\geqslant 2$.

Maybe density being quasi-concave is enough to guarantee monotonicity? All positive examples are quasi-concave. All negative examples are not quasi-concave.

==> ROC_table.tex <==
\newcommand{\myro}[3]{ #1 & #2 & #3 \\ \hline}
\begin{table}[!h]
	\label{tab:compare}
	\centering
	\begin{tabular}{|c|c|c|}
	\hline
	\myro{Mechanism}{Privacy}{$\E X^2\big/\ep^{-2}$}
	\myro{Gaussian}{$\ep$-GDP}{$1$}
	\myro{TGU}{$(\ep,0)$-DP}{$2-O(\ep^2)$}
	\myro{Laplace}{$(\ep,0)$-DP}{$2$}
	\myro{Truncated Laplace}{$(\ep,\delta)$-DP}{$2-O(\ep^2)$}
	\myro{Gaussian}{$(\ep,\delta)$-DP}{$2\log(1.25\delta^{-1})$}
	\end{tabular}
\end{table}

% \begin{table}[!h]
% 	\label{tab:compare}
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% 	\hline
% 	\myro{Mechanism}{Privacy}{$\E X^2\big/\ep^{-2}$}
% 	\myro{Gaussian}{$\ep$-GDP}{$1$}
% 	\myro{Double Geometric}{$(\ep,0)$-DP}{$2-O(\ep^2)$}
% 	\myro{Laplace}{$(\ep,0)$-DP}{$2$}
% 	\myro{Truncated Laplace}{$(\ep,\delta)$-DP}{$2-O(\ep^2)$}
% 	\myro{Gaussian}{$O(\ep)$ better than $(\ep,\delta)$-DP}{$2\log(1.25\delta^{-1})$}
% 	\end{tabular}
% \end{table}

% \begin{table}[!h]
% 	\label{tab:compare}
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% 	\hline
% 	\myro{Mechanism}{Privacy}{$\E X^2\big/\ep^{-2}$}
% 	\myro{Gaussian}{$\ep$-GDP}{$1$}
% 	\myro{Double Geometric}{$(\ep,0)$-DP$}{$2-O(\ep^2)$}
% 	\myro{Laplace}{$(\ep,0)$-DP+O(\ep^2)$}{$2$}
% 	\myro{Truncated Laplace}{$(\ep,\delta)$-DP^2)$}{$2-O(\ep^2)$}
% 	\myro{Gaussian}{$(\ep,\delta)$-DP)$}{$2\log(1.25\delta^{-1})$}
% 	\end{tabular}
% \end{table}

==> algo.tex <==
\section{A New Query Answering Algorithm with Small $\ell_\infty$ Error} % (fold)
\label{sec:a_new_algorithm_for_}



\begin{algorithm}[htb]
	\caption{\texttt{Private Query Answering with Samll $\ell_\infty$ error}}\label{algo:inf}
	\begin{algorithmic}[1]
	\State{\bf Input:} Dataset $D$, target function $f$, dimension $n$, privacy parameter $\mu$.
	\State{\bf Output:} Private estimation $M(D)$
		\State Let $p=2\log\log n$
		\State Sample $X$ with density $\propto\e^{-\sum |x_i|^p}$ with $\alpha=p=2\log\log n$
		\State Let $t=\sens(f)\cdot \sqrt{\|\Fisher_{p,p}\|_2/\mu}=\sens(f)\cdot \sqrt{p^2\cdot\frac{1}{\mu}\cdot\frac{\Gamma(2-\frac{1}{p})}{\Gamma(\frac{1}{p})}}$
		\State Return $M(D)=f(D)+t X$
	\end{algorithmic}
\end{algorithm}
There is a simple and effcient algorithm that samples $X$ with density $\propto\e^{-\sum |x_i|^p}$ for arbitrary $p\in[1,+\infty]$. We achieve this by generalizing the approach in \cite{HardtTa10}, which focuses on $\alpha=1$, and the uniform sampler of the $\ell_p$ unit ball, which appears in \cite{calafiore1998uniform}. Unfortunately due to the page limit, we have to relegate this algorithm to the appendix.
\begin{restatable}[]{theorem}{inferr}
\label{thm:infinity_error}
	The mechanism $M$ in \Cref{algo:inf} is asymptotically $\mu$-GDP for most $D,D'$ and $f$, and with probability at least $1-\delta$,
	\[\|M(D)-f(D)\|_\infty\leqslant C\cdot \sens(f)\cdot \sqrt{\log\log n}\cdot (\log\delta^{-1})^{\frac{1}{2\log\log n}}\]
	where $C$ is a universal constant.
\end{restatable}
In particular, when $\delta\geqslant n^{-c}$ for some $c>0$, the factor that involves $\delta$ becomes a constant, so the error is bounded by $O(\sens(f)\cdot \sqrt{\log\log n})$. Note that in order to have $\log \log n >1$ it suffices to take $n>15$. A particularly interesting use case of this theorem is when each dimension of $f$ is a one-way marginal (fraction of the population with certain traits). In this case each dimension has sensitivity $\frac{1}{N}$ where $N$ denotes the size of the dataset $D$. Hence $\sens(f)=\frac{\sqrt{n}}{N}$ and the error is 
	$O(\frac{1}{N}\sqrt{n\log\log n})$, which recovers the result in \cite{SteinkeUl17}.


If the (trivial) uncertainty principle \eqref{eq:newCR} is tight, which means there exist $n$-dimensional distributions $X_{\varphi_n}$ such that $\E\|X_{\varphi_n}\|_2^2\cdot\|\Fisher_{\varphi_n}\|_2=O(1)$, then the algorithm can be further improved, answering an open question proposed by the authors of \cite{SteinkeUl17} in the affirmative, which leads to attractive bounty in the form of food.

% section a_new_algorithm_for_ (end)


==> budget.tex <==
\newcommand{\Lap}{\mathrm{Lap}}
\section{How to Fully Exploit Your Privacy Budget} % (fold)
\label{sec:how_to_fully_exploit_your_privacy_budget}
All known algorithms for private mean estimation look like $M(S) = \hat{\theta}(S)+\xi$ where $\xi\sim P$. By ``privacy budget'' we mean the specific privacy notion that we hope $M$ satisfy. Moreover, we focus on privacy notions within $f$-DP framework. Three most interesting notions are 
\begin{enumerate}
	\item $(\ep,0)$-DP, i.e. $f_{\ep,0}$-DP in the language of $f$-DP;
	\item $(\ep,\delta)$-DP, i.e. $f_{\ep,\delta}$-DP in the language of $f$-DP;
	\item $\mu$-GDP, i.e. $G_\mu$-DP in the language of $f$-DP.
\end{enumerate}

\subsection{1-dim} % (fold)
\label{sub:1_dim}
Assume the sensitivity of $\hat{\theta}$ is $t$, then for neighboring datasets $S,S'$, adversary faces the testing of $P$ vs $P+t$ where $P+t$ refers to the law of $\xi+t$ when $\xi\sim P$. Fully exploiting privacy budget means to find $P$ such that $T(P,P+t)=f_{\ep,0}, f_{\ep,\delta}$ and $G_\mu$ respectively.
\begin{enumerate}
	\item When $P=N(0,\frac{t^2}{\mu^2})$, $T(P,P+t)=G_\mu$.

	When $\xi\sim P$, $\E\xi^2 = \frac{t^2}{\mu^2}$.
	\item When $P = t\cdot \mathrm{DGeom}(p)$ where $p=\e^{-\ep}$, $T(P,P+t)=f_{\ep,0}$. Note that if $\xi\sim\mathrm{DGeom}(p)$ then $\xi = n$ w.p. $\frac{1}{Z}p^{-|n|}$. Easy calculation shows $Z = \frac{1-p}{1+p}$. The discrete nature of DGeom makes it hard to extend the application beyond counting query. Maybe Ilya Mironov or someone else has something to say.

	Alternatively, When $P = \frac{t}{\ep}\cdot \Lap(0,1)$, $T(P,P+t)\approx f_{\ep,0}$.

	When $\xi\sim P$, $\E\xi^2 = \frac{2t^2}{\ep^2}$.
	\item For $h>0$, let $\Lap^h$ be standard Laplace truncated at $\pm h$.
	\begin{lemma}[Informal]
	When $P= \frac{t}{\ep}\cdot \Lap^h(0,1)$ and $h=\log (1+\frac{\e^\ep-1}{2}\cdot \delta^{-1})$,
	$T(P,P+t) \approx f_{\ep,\delta}$.
	\end{lemma}
	If you are familiar with $f$-DP technique, you may guess that $T(P,P+t)= T(\Lap, \Lap+1)\otimes f_{0,\delta}$, but this is not true.
	\begin{lemma} \label{lem:}
		\djs{Not 100\% sure} When $\xi\sim P$ as in the above lemma,
		\begin{align*}
			\E\xi^2 &= \frac{2-\e^{-h}(h^2+2h+2)}{1-\e^{-h}}.
		\end{align*}
	\end{lemma}
\end{enumerate}

Suppose $f=T(P,P+t)$ where $P$ is log-concave, with cdf $F$. Then $f(\alpha) = F(F^{-1}(1-\alpha)-t)$. Let $P^h$ be $P$ after $\pm h$ truncation. Its cdf is
\[F^h(x) = \frac{F(x)-F(-h)}{F(h)-F(-h)}\Big[^1_0\]
where $\Big[^1_0$ means truncating at 0 and 1. $P^h$ is still log-concave. Let's find $f^h = T(P^h,P^h+t)$. For the rejection region $\{x>a\}$, its type I and type II error are
\begin{align*}
	\alpha &= 1-F^h(a) = 1-\frac{F(a)-F(-h)}{F(h)-F(-h)}\Big[^1_0\\
	\beta &= F^h(a-t) =\frac{F(a-t)-F(-h)}{F(h)-F(-h)}\Big[^1_0
\end{align*}
Ignore truncation at 0 and 1 for now. Let $Z = F(h)-F(-h)$. Then
\begin{align*}
	1-F(a) &= Z\alpha+1-F(h)\\
	F(a-t)&=Z\beta+F(-h)
\end{align*}
That is, if $\beta = f^h(\alpha)$, then
\begin{align*}
	Z\beta+F(-h) = f(Z\alpha+1-F(h)).
\end{align*}
Ideally we want to find $P$ and $h$ such that $f^h = f_{\ep,\delta}$. To start let's find an approximate version first. Let $P=\Lap$. We have $F(-h)=\frac{1}{2}\e^{-h}$ and $Z = 1-\e^{-h}$.

A necessary condition for $f^h=f_{\ep,\delta}$ is $f^h(0)=1-\delta$. Now that we have fixed $P=\Lap$, this leads us to the expression of $h$. The resulting $f^h$ mostly agrees with $f_{\ep,\delta}$. The following lemma precisely describes this property.
\begin{lemma} \label{lem:}
	Let $P= \frac{t}{\ep}\cdot \Lap^h(0,1)$ and $h=\log (1+\frac{\e^\ep-1}{2}\cdot \delta^{-1})$. Let
	$f^h=T(P,P+t)$. Then
	\[f^h(\alpha)=f_{\ep,\delta}(\alpha)\text{ for } \alpha\not\in[\e^{-\ep}(\tfrac{1}{2}-\delta),\tfrac{1}{2}].\]
	In that interval, $f^h$ satisfies a translated reciprocal function, namely,
	\begin{align*}
		\big((1-\e^{-h})f^h(\alpha)+\frac{1}{2}\e^{-h}\big)\cdot \big((1-\e^{-h})\alpha+\frac{1}{2}\e^{-h}\big) = \frac{\e^{-\ep}}{4}.
	\end{align*}
	% \begin{align*}
	% 	f^h(\alpha) = \left\{
	% 	\begin{array}{ll}
	% 	, 		& \text{if } 0<n<k, \\
	% 	f_{\ep,\delta}(\alpha), 		& \text{otherwise }
	% 	\end{array}
	% 	\right.
	% \end{align*}
\end{lemma}
\subsection{Gaussian vs Truncated Laplace for $(\ep,\delta)$-DP} % (fold)
\label{sub:gaussian_vs_truncated_laplace}
We compare four mechanisms, all have the form 
$\hat{\theta}(S)+\xi$.
\begin{enumerate}
	\item Laplace mechanism (Lap): $\xi\sim\frac{t}{\ep}\cdot \Lap(0,1)$.
	\item Old Gaussian mechanism ($G_{2006}$): $\xi\sim N(0,\frac{2t^2\log(1.25\delta^{-1})}{\ep^2})$.
	\item Truncated Laplace mechanism (T-Lap): $\xi\sim \frac{t}{\ep}\cdot \Lap^h(0,1)$ and $h=\log (1+\frac{\e^\ep-1}{2}\cdot \delta^{-1})$
	\item New Gaussian mechanism ($G_{2019}$): $\xi\sim N(0,\frac{t^2}{\ep^2})$.
\end{enumerate}
\begin{table}[!h]
	\label{tab:compare}
	\centering
	\begin{tabular}{|c|c|c|}
	\hline
	 & Privacy & $\E\xi^2\big/\frac{t^2}{\ep^2}$ \\ \hline
	Lap & $(\ep,0)$-DP & 2 \\ \hline
	$G_{2006}$ & $(\ep,\delta)$-DP & $2\log(1.25\delta^{-1})$ \\ \hline
	T-Lap &  $(\ep,\delta)$-DP & $<2$ \\ \hline
	$G_{2019}$ &  $\ep$-GDP & 1 \\ \hline
	\end{tabular}
\end{table}
% subsection gaussian_vs_truncated_laplace (end)
% section how_to_fully_exploit_your_privacy_budget (end)


==> empirical_general.tex <==

\paragraph{Empirical Trade-off Function} 
\label{par:empirical_trade_off_function}

% paragraph empirical_trade_off_function (end)
For a given mechanism $M$ and neighboring inputs $D$ and $D'$, it is often hard to evaluate $T\big(M(D),M(D')\big)$ exactly. One source of difficulty is that for complicated mechanism, it is already quite hard to compute the density of the distributions $M(D)$ and $M(D')$. \cite{dong2019gaussian} developed some tools such as composition and subsampling, but the general problem still exists.

As we will justify later, we are often blessed with simple yet optimal mechanisms. In this case even though the density can be easily evaluated, the likelihood ratio test can still yield a complicated rejection region, especially when the dimension is high. This suggests the Monte Carlo method to estimate $T\big(M(D),M(D')\big)$. We elaborate the details below.

Let $X$ and $X'$ be random variables with distributions $M(D)$ and $M(D')$ respectively, and let $p(x)$ and $p'(x)$ be the corresponding densities. We know the log likelihood ratio is $\log p'(x)-\log p(x)$. Thresholding it at $h$ yields the following type I and type II errors
\begin{align*}
    \alpha(h) &= \P(\log p'(X)-\log p(X)>h)\\
    \beta(h) &= \P(\log p'(X')-\log p(X')\leqslant h)
\end{align*}
Once we have these, $T\big(M(D),M(D')\big)$ can be obtained by eliminating $h$ and express $\beta$ as a function of $\alpha$. These two probabilities can be computed by a simple Monte Carlo approach. First we  generate $\{x_1,\ldots, x_N\}$ and $\{x_1',\ldots, x_N'\}$, which are i.i.d. copies of $X$ and $X'$. Let
\begin{align*}
    a_i &= \log p'(x_i)-\log p(x_i)\\
    b_i &= \log p'(x_i')-\log p(x_i')\\
    \hat{\alpha}(h) &= \frac{1}{N} \cdot\#\{a_i>h\}\\
    \hat{\beta}(h) &= \frac{1}{N}\cdot \#\{b_i\leqslant h\}
\end{align*}
We only evaluate on a discrete set of $h$ such that the corresponding $\alpha$ forms a uniform grid $\{\frac{1}{N},\ldots, \frac{N}{N}\}$. Let $h_j = a_{(N-j)}$ where $a_{(1)}\leqslant\cdots \leqslant a_{(N)}$ are order statistics of $a_i,i=1,2,\ldots, N$. We further assume $a_{(0)}=-\infty$. Then for $j=0,1,2,\ldots, N$,
\begin{align*}
     \hat{\alpha}_j &= \hat{\alpha}(h_j)=\frac{1}{N}\cdot \#\{a_i> a_{(N-j)}\}=\frac{j}{N}\\
     \hat{\beta}_j &= \hat{\beta}(h_j) = \frac{1}{N}\cdot \#\{b_i\leqslant a_{(N-j)}\}
\end{align*}
Let $\hat{T}_N\big(M(D),M(D')\big)$ be the function that linearly interpolates the values $\hat{\beta}_0,\ldots, \hat{\beta}_N$ at $\frac{0}{N},\ldots, \frac{N}{N}$. As a direct consequence of the well-known Glivenko–Cantelli theorem, we have
\[\|\hat{T}_N\big(M(D),M(D')\big)-T\big(M(D),M(D')\big)\|_\infty
% =\sup_{\alpha\in[0,1]}|\hat{T}_N\big(M(D),M(D')\big)(\alpha)-T\big(M(D),M(D')\big)(\alpha)|
\to 0 \text{ almost surely.}\] 

% subsection details_of_empirical_trade_off_functions (end)


==> inf_norm_table.tex <==
\begin{table*}[!t]
	\caption{Explicit expressions for the $\ell_\infty$ uncertainty principle.}\label{tab:compare_inf}
	\centering
	\begin{tabular}{|c|c|c|c|}
	\hline
	% _{p,\alpha}
	 Density & $\E\|X\|_\infty^2$ & $\|\Fisher_\varphi\|_2$ & $\E\|X\|_\infty^2\cdot{\|\Fisher_\varphi\|_2}$\\ \hline
	% $\propto \e^{-\|x\|_1}$ & $2n$ & $I$ & $2n$\\ \hline
	% $\propto \e^{-\|x\|_2}$ & $n(n+1)$ & $\frac{1}{n}I$ & $n+1$\\ \hline
	% $\propto \e^{-\|x\|_2^2}$ & $\frac{1}{2}n$ & $2I$ & $n$\\ \hline
	% $\propto \e^{-\|x\|_\infty}$ & $\frac{1}{3}n(n+1)(n+2)$ & $\frac{1}{n}I$ & $\frac{1}{3}(n+1)(n+2)$\\ \hline
	$\propto \e^{-\|x\|_1^\alpha}$ & $\sim\left(\frac{n}{\alpha}\right)^{\frac{2}{\alpha}}\cdot\left(\frac{{\log n}}{n}\right)^2$ & $\sim n^{2}\cdot \left(\frac{\alpha}{n}\right)^{\frac{2}{\alpha}}$ & $\sim ({\log n})^2$\\ \hline
	$\propto \e^{-\|x\|_2^\alpha}$ & $\sim\left(\frac{n}{\alpha}\right)^{\frac{2}{\alpha}}\cdot{\frac{2\log n}{n}}$ & $\sim n\cdot \left(\frac{\alpha}{n}\right)^{\frac{2}{\alpha}}$ & $\sim {2{\log n}}$\\ \hline
	$\propto \e^{-\|x\|_p^\alpha}$ & $O_p\left(\left(\frac{n}{\alpha}\right)^{\frac{2}{\alpha}}\cdot\left({\frac{\log n}{n}}\right)^{\frac{2}{p}}\right)$ & $O_p\left(n^{\frac{2}{p}}\cdot \left(\frac{\alpha}{n}\right)^{\frac{2}{\alpha}}\right)$ & $O_p\big((\log n)^{\frac{2}{p}}\big)$\\\hline
	% $\propto \e^{-\|x\|_\infty^\alpha}$ & $\sim\left(\frac{n}{\alpha}\right)^{\frac{1}{\alpha}}$ & $\sim\alpha^{\frac{2}{\alpha}}\cdot  n^{1-\frac{2}{\alpha}}$ & $\sim \sqrt{n}$\\ \hline
	\end{tabular}
	% \vspace{1em}
	% \vspace{-1.5em}
\end{table*}

==> infinity.tex <==
$X_i\sim U[-1,1]$
\begin{align*}
	g(t)=\P(|X_i+\frac{1}{n}|<t) = 
			\left\{
			\begin{array}{ll}
			\frac{t+1-\frac{1}{n}}{2}, & t\in(1-\frac{1}{n},1+\frac{1}{n})\\
			t, &t\in(0,1-\frac{1}{n}).
			\end{array}
			\right.
\end{align*}
\begin{align*}
	\E\|U+\frac{1}{n}v\|_{\infty} &= \E\max|X_i+\frac{1}{n}|\\
	&=\int_0^{1+\frac{1}{n}}\P(|X_i+\frac{1}{n}|>t)\diff t\\
	&=\int_0^{1+\frac{1}{n}}1-g^n(t)\diff t\\
	&=\int_0^{1-\frac{1}{n}}1-t^n\diff t
	+\int_{1-\frac{1}{n}}^{1+\frac{1}{n}}1-\left(\frac{t+1-\frac{1}{n}}{2}\right)^n\diff t\\
	&=1-\frac{1}{n}-\frac{1}{n+1}\left(1-\frac{1}{n}\right)^{n+1}+\frac{2}{n}
	-2\int_{1-\frac{1}{n}}^{1+\frac{1}{n}}\left(\frac{t+1-\frac{1}{n}}{2}\right)^n\diff \left(\frac{t+1-\frac{1}{n}}{2}\right)\\
	&=1+\frac{1-\e^{-1}}{n}-\frac{2}{n+1}(1-\left(1-\frac{1}{n}\right)^{n+1})+o(\frac{1}{n})\\
	&=1+\frac{1-\e^{-1}}{n}-\frac{2(1-\e^{-1})}{n}+o(\frac{1}{n})\\
	&=1-\frac{1-\e^{-1}}{n}+o(\frac{1}{n})
\end{align*}
\begin{align*}
	\E\|U+\frac{1}{n}v\|_{\infty}^2 &= \E\max|X_i+\frac{1}{n}|^2\\
	&=\int_0^{(1+\frac{1}{n})^2}\P(|X_i+\frac{1}{n}|^2>t)\diff t\\
	&=\int_0^{(1+\frac{1}{n})^2}1-g^n(\sqrt{t})\diff t\\
	&=\int_0^{1+\frac{1}{n}}(1-g^n(t))2t\diff t\\
	&=\underbrace{\int_0^{1-\frac{1}{n}}2t(1-t^n)\diff t}_{I_1}
	+\underbrace{\int_{1-\frac{1}{n}}^{1+\frac{1}{n}}\left(1-\left(\frac{t+1-\frac{1}{n}}{2}\right)^n\right)\cdot 2t\diff t}_{I_2}\\
	I_1&=\left(1-\frac{1}{n}\right)^2-\int_0^{1-\frac{1}{n}}2t^{n+1}\diff t\\
	&=\left(1-\frac{1}{n}\right)^2-\frac{2}{n+2}\left(1-\frac{1}{n}\right)^{n+2}=1-\frac{2}{n}-\frac{1}{n}\cdot\frac{1}{\e}+o(\frac{1}{n})\\
	I_2&=\left(1+\frac{1}{n}\right)^2-\left(1-\frac{1}{n}\right)^2
	-\int_{1-\frac{1}{n}}^{1+\frac{1}{n}}\left(\frac{t+1-\frac{1}{n}}{2}\right)^n\cdot 2t\diff t\\
	\int_{1-\frac{1}{n}}^{1+\frac{1}{n}}\left(\frac{t+1-\frac{1}{n}}{2}\right)^n\cdot 2t\diff t&=
	\int_{1-\frac{1}{n}}^{1+\frac{1}{n}}\left(\frac{t+1-\frac{1}{n}}{2}\right)^n\cdot 4\left(\frac{t+1-\frac{1}{n}}{2}-\frac{1-\frac{1}{n}}{2}\right)\diff t\\
	&=4\int_{1-\frac{1}{n}}^{1+\frac{1}{n}}\left(\frac{t+1-\frac{1}{n}}{2}\right)^{n+1}\diff t
	-2\left(1-\frac{1}{n}\right)\int_{1-\frac{1}{n}}^{1+\frac{1}{n}}\left(\frac{t+1-\frac{1}{n}}{2}\right)^n\diff t\\
	&=\frac{8}{n+2}\left(\frac{t+1-\frac{1}{n}}{2}\right)^{n+2}\bigg|_{1-\frac{1}{n}}^{1+\frac{1}{n}}
	-2\left(1-\frac{1}{n}\right)\cdot\frac{1}{n+1}(1-\e^{-1})\\
	&=\frac{8}{n}(1-\e^{-1})-\frac{2}{n}(1-\e^{-1})+o(\frac{1}{n})\\
	\E\|U+\frac{1}{n}v\|_{\infty}^2
	&=I_1+I_2\\
	&=1-\frac{2+\e^{-1}}{n}+\frac{6}{n}(1-\e^{-1})+o(\frac{1}{n})\\
	&=1+\frac{4-7\e^{-1}}{n}+o(\frac{1}{n})
	\end{align*}

==> numerical.tex <==
\section{Numerical Evidences} % (fold)
\label{sec:numerical_evidences}

% section numerical_evidences (end)
Computing Levy distance
$L(F,\Phi) = \min \{t:\Phi(x-t)-t\leqslant F(x)\leqslant \Phi(x+t)+t, \forall x\in\R\}$.
In particular, let $-\infty=x_0\leqslant x_1\leqslant \cdots \leqslant x_n\leqslant x_{n+1}=+\infty$, then $F(x) = k/n, x\in[x_k,x_{k+1}), k=0,1,\ldots, n$
It suffices that the $\Phi$ translation be below the left limit and above the right limit at each $x_k$, i.e.
$$\Phi(x_k-t)-t\leqslant F(x_k-0)\leqslant F(x_k+0)\leqslant \Phi(x+t)+t$$
$$\Phi(x_k-t)-t\leqslant \frac{k-1}{n}, \frac{k}{n} \leqslant \Phi(x_k+t)+t$$
We first present the algorithm that samples an $n$-dimensional random vector whose density is $\propto\e^{-\|x\|_p^\alpha}$.

\begin{algorithm}[htb]
	\caption{\texttt{Sample $\propto\e^{-\|x\|_p^\alpha}$}}\label{algo:sample}
	\begin{algorithmic}[1]
	\State{\bf Input:} $p,\alpha$ and dimension $n$
        % xi = scipy.stats.gamma.rvs(1/p, size=d)
        % xi = xi**(1/p)
        % xi = np.multiply(xi, scipy.stats.bernoulli.rvs(.5,size=d)*2-1)
        % w = scipy.stats.uniform.rvs(0,1)
        % return w**(1/d)*xi/norm(xi,p)
		% \State {\bf Subsampling:}
		\Statex Generate $t\sim \Gamma(\frac{n}{\alpha}+1,1)$
		\Statex Generate $\xi_i,i=1,2,\ldots, n$ i.i.d. from $\Gamma(\frac{1}{p},1)$
		\Statex Generate random vector $\bm x\in\R^n$ where $x_i=\epsilon_i\cdot\xi_i^{\frac{1}{p}}$, $\epsilon_i$ are Rademacher random variables (unbiased coin flips) independent from everything else.
		\Statex Generate $r\sim U[0,1]$
		\Statex Let $V=r^{\frac{1}{n}}\cdot \frac{x}{\|x\|_p}$
		% \State {\bf Average, perturb, and descend:}
		% \Statex \hspace{0.55cm} {$\theta_{t+1} \gets \theta_{t} - \eta_t \Big(\frac{1}{m} \sum_i\bar{v}_t^{(i)}+\N(0, \frac{4\sigma^2 C^2}{m^2} I)\Big)$}
                 % \Comment{$I$ is an identity matrix}
		\State {\bf Output} $t\cdot V$
%\bmnote{Ref to Eqs or pseudocode for computing privacy cost.}
%LZ: we will spend most of time discussing how privacy is computed. Since
%the algorithm description is an outline, maybe we can postpone it?
	\end{algorithmic}
\end{algorithm}
It is easy to see its correctness from \Cref{thm:uniform} and \cite{calafiore1998uniform}. The special case of $p=\alpha$, thanks to indepence of the coordinates, has an even simpler implementation as in \Cref{algo:simple}.
\begin{algorithm}[!h]
	\caption{\texttt{Sample $\propto\e^{-\sum|x_i|^p}$}}\label{algo:simple}
	\begin{algorithmic}[1]
	\State{\bf Input:} $p$ and dimension $n$
		\Statex Generate $\xi_i,i=1,2,\ldots, n$ i.i.d. from $\Gamma(\frac{1}{p},1)$
		\Statex Generate random vector $\bm x\in\R^n$ where $x_i=\epsilon_i\cdot\xi_i^{p}$, $\epsilon_i$ are Rademacher random variables (unbiased coin flips) independent from everything else.
		\State {\bf Output} $\bm x$
	\end{algorithmic}
\end{algorithm}

